Multi-Level Languages are Generalized Arrows

Multi-level languages and Arrows both facilitate metaprogramming, the act of writing a program which generates a program. The arr function required of all Arrows turns arbitrary host language expressions into guest language expressions; because of this, Arrows may be used for metaprogramming only when the guest language is a superset of the host language. This restriction is also present in multi-level languages which offer unlimited cross-level persistence. <p> This paper introduces generalized arrows and proves that they generalize Arrows in the following sense: every Arrow in a programming language arises from a generalized arrow with that language's term category as its codomain. Generalized arrows impose no containment relationship between the guest language and host language; they facilitate heterogeneous metaprogramming. The category having all generalized arrows as its morphisms and the category having all multi-level languages as its morphisms are isomorphic categories. This is proven formally in Coq, and the proof is offered as justification for the assertion that multi-level languages are generalized arrows. <p> Combined with the existence of a particular kind of retraction in the host language, this proof can be used to define an invertible translation from two-level terms to one-level terms parameterized by a generalized arrow instance. This is ergonomically significant: it lets guest language providers write generalized arrow instances while the users of those guest languages write multi-level terms. This is beneficial because implementing a generalized arrow instance is easier than modifying a compiler, whereas writing two-level terms is easier than manipulating generalized arrow terms.

==> megacz-tilde.inc <==
% verbatim with realigned tilde %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{verbatim}
\usepackage{fancyvrb}
\def\tild{\rlap{\lower.85ex\hbox{\large\char126}}\ }
\DefineVerbatimEnvironment%
 {verbatim}%
 {Verbatim}%
 {codes={\catcode`~=\active}%
 ,samepage=true%
 ,defineactive=\def~{\tild}%
 }
\DefineVerbatimEnvironment%
 {verbatimWithCommands}%
 {Verbatim}%
 {codes={\catcode`~=\active}%
 ,samepage=true%
 ,defineactive=\def~{\tild}%
 ,commandchars=\\\{\}%
 }
\DefineVerbatimEnvironment%
 {verbatimsm}%
 {Verbatim}%
 {codes={\catcode`~=\active},%
  samepage=true,
  fontsize=\small,
  defineactive=\def~{\tild}%
 }


